A Generalized Framework for Microstructural Optimization using Neural Networks

Microstructures, i.e., architected materials, are designed today, typically, by maximizing an objective, such as bulk modulus, subject to a volume constraint. However, in many applications, it is often more appropriate to impose constraints on other physical quantities of interest. In this paper, we consider such generalized microstructural optimization problems where any of the microstructural quantities, namely, bulk, shear, Poisson ratio, or volume, can serve as the objective, while the remaining can serve as constraints. In particular, we propose here a neural-network (NN) framework to solve such problems. The framework relies on the classic density formulation of microstructural optimization, but the density field is represented through the NN's weights and biases. The main characteristics of the proposed NN framework are: (1) it supports automatic differentiation, eliminating the need for manual sensitivity derivations, (2) smoothing filters are not required due to implicit filtering, (3) the framework can be easily extended to multiple-materials, and (4) a high-resolution microstructural topology can be recovered through a simple post-processing step. The framework is illustrated through a variety of microstructural optimization problems.

==> abstract.tex <==
\begin{abstract}
	Multiscale topology optimization (M-TO) entails generating an optimal global topology, together with an optimal set of microstructures at a smaller scale, for a physics constrained problem. With the advent of additive manufacturing, M-TO has gained significant prominence. However, generating  distinct and optimal microstructures  at various  locations can be computationally very expensive. As an alternate, \emph {graded multiscale topology optimization} (GM-TO) has been proposed where one or more pre-selected and graded (parameterized) microstructural topologies are used to optimally fill the domain. This leads to significant reduction in computation, while retaining many of the benefits of M-TO.
	
	A successful GM-TO framework must: (1) be capable of efficiently handling numerous pre-selected microstructures, (2) be able to continuously switch between these  microstructures (during optimization), (3) ensure that the partition of unity is satisfied, and (4) discourage microstructure mixing at termination.
	
	In this paper, we propose to meet these requirements by exploiting the unique classification capacity of neural networks. Specifically, we propose a \emph {graded multiscale topology optimization using neural-network} (GM-TOuNN) framework with the following features: (1) the number of design variables is only weakly dependent on the number of pre-selected microstructures, (2) it guarantees partition of unity, while discouraging microstructure mixing, and (3) it supports automatic differentiation, thereby  eliminating manual sensitivity analysis. The proposed framework is illustrated through several examples.

{\centering
\includegraphics[scale=0.6]{Figures/Method/graphicalAbstract.pdf}
\captionof*{figure}{Overview of the proposed method: Given candidate microstructures and a topology optimization problem, a neural network (NN) maps the spatial coordinates to a volume fraction field and a microstructure field, that produce a graded multiscale design.}
\par
}
\end{abstract}
